Improved Communication Complexity of Fault-Tolerant Consensus

Consensus is one of the most thoroughly studied problems in distributed computing, yet there are still complexity gaps that have not been bridged for decades. In particular, in the classical message-passing setting with processes' crashes, since the seminal works of Bar-Joseph and Ben-Or [1998] \cite{Bar-JosephB98} and Aspnes and Waarts [1996, 1998] \cite{AspnesW-SICOMP-96,Aspnes-JACM-98} in the previous century, there is still a fundamental unresolved question about communication complexity of fast randomized Consensus against a (strong) adaptive adversary crashing processes arbitrarily online. The best known upper bound on the number of communication bits is $\Theta(\frac{n^{3/2}}{\sqrt{\log{n}}})$ per process, while the best lower bound is $\Omega(1)$. This is in contrast to randomized Consensus against a (weak) oblivious adversary, for which time-almost-optimal algorithms guarantee amortized $O(1)$ communication bits per process \cite{GK-SODA-10}. We design an algorithm against adaptive adversary that reduces the communication gap by nearly linear factor to $O(\sqrt{n}\cdot\text{polylog } n)$ bits per process, while keeping almost-optimal (up to factor $O(\log^3 n)$) time complexity $O(\sqrt{n}\cdot\log^{5/2} n)$. More surprisingly, we show this complexity indeed can be lowered further, but at the expense of increasing time complexity, i.e., there is a {\em trade-off} between communication complexity and time complexity. More specifically, our main Consensus algorithm allows to reduce communication complexity per process to any value from $\text{polylog } n$ to $O(\sqrt{n}\cdot\text{polylog } n)$, as long as Time $\times$ Communication $= O(n\cdot \text{polylog } n)$. Similarly, reducing time complexity requires more random bits per process, i.e., Time $\times$ Randomness $=O(n\cdot \text{polylog } n)$.

==> src/lower_bound.tex <==
\section{A Lower Bound}
In asynchronous networks there is a lower bound showing that, for any $t$-resilient randomized \textit{asynchronous} Consensus algorithm, there exists an adversarial strategy that enforces the algorithm to use at least $\Omega(n/\log n)$ messages per process, with high probability. We cannot expect this result to hold in \textit{synchronous} networks because of our \ParamConsensus{} algorithm breaking the $\Theta(n/\log n)$ barrier. However, we can make a connection between the number of rounds used by any (even synchronous) randomized algorithm, which must be $\Omega(\sqrt{n/\log n})$ by~\cite{Bar-JosephB98}, and the amortized number of messages sent (or the number of rounds with random choices made) by a process running any given Consensus algorithm against an adaptive adversary. We aim at the following result. 


%\begin{definition}
%An algorithm is \textit{} if i  
%\end{definition}

\begin{theorem}
\label{thm:lower-randomness}
For any randomized algorithm solving Consensus in time $\tau = \Omega(\sqrt{n/\log n})$ with a constant probability against an adaptive adversary, there is an adaptive 
%fail-stop $t$-adversary 
adversary
which can force the algorithm to have $\Omega(\min\{\frac{n}{\tau\log n},\tau\})$ rounds with use of randomness, amortized per process, with a constant probability.
%the product of the number of messages used and the number of rounds being at least $\Omega(\frac{n^2}{\polylog n})$ with high probability.
\end{theorem}

The proof of Theorem~\ref{thm:lower-randomness} is given in the following Section~\ref{sec:proof-lower}.

Theorem~\ref{thm:lower-randomness} implies a lower bound on the number of messages for a certain class of algorithms.
Consider a class of algorithms in which a process that does not communicate (i.e., send or receive a message) with any other process in a round does not use randomness in that round. We call this class {\em sleeping algorithms}.
%It follows from Theorem~\ref{thm:lower-randomness} that sleeping algorithms cannot have lower communication than $\Omega(\min\{\frac{n}{\tau\log n}+1,\tau\})$ bits per process.

\begin{theorem}
\label{thm:lower-communication}
For any 
%randomized 
sleeping
algorithm solving Consensus in time $\tau = \Omega(\sqrt{n/\log n})$ with a constant probability against an adaptive adversary, there is an 
%adaptive 
%%%%%fail-stop $t$-adversary 
%adversary
adversarial strategy
which can force the algorithm to use $\Omega(\min\{\frac{n}{\tau\log n}+1,\tau\})$ 
messages (and thus, also communication bits), amortized per process.
%the product of the number of messages used and the number of rounds being at least $\Omega(\frac{n^2}{\polylog n})$ with high probability.
\end{theorem}

\begin{proof}
Otherwise, for every adversarial strategy, any constant $c>0$ and a constant probability $q>0$, the number of communication bits amortized per process would be smaller than $c\cdot \min\{1,\frac{n}{\tau\log n},\tau\}$ with probability $q$. Hence, by definition of the class of sleeping algorithms, $c\cdot \min\{1,\frac{n}{\tau\log n},\tau\}$ would also be an upper bound on the number of rounds using randomness, amortized per process, with probability $q$, for any adversarial strategy. It however contradicts Theorem~\ref{thm:lower-randomness}.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:lower-randomness}}
\label{sec:proof-lower}

Consider a randomized algorithm solving Consensus in time $\tau = \Omega(\sqrt{n/\log n})$ with a constant probability against an adaptive adversary. We adjust the ideas in the proof of the lower bound $\Omega\left(\sqrt{\frac{n}{\log n}}\right)$ on the number of rounds from \cite{Bar-JosephB98} to our analysis of the number of processes' rounds with use of randomness.

\paragraph{Preliminaries.}

In~\cite{Bar-JosephB98}, the main probabilistic tool was a coin flipping game: \dk{To Be Described in More Details.} 
%was considered and 
The following result was proved:\footnote{Here we give more general version, as in the original proof $\alpha$ was at some point fixed to $1/n$, in order to formulate a result needed in that paper; but the arguments holds for any $2^{m/(16k^2)}<\alpha\le 1/2$.} 

\begin{corollary}[Corollary 2.2 in~\cite{Bar-JosephB98}]
\label{cor:coin-game}
For sufficiently large $m$ and any $2^{m/(16k^2)}<\alpha\le 1/2$, in an $m$ player one round coin flipping game with $k$ possible outcomes, 
if the adversary can crash more than $4k\sqrt{m\log \alpha^{-1}}$ players, he can bias the result towards one particular outcome with probability greater than $1-\alpha$.
\end{corollary}

We will also use this result to bias an execution of the algorithm towards undecided state (so called null-valent) with probability at least $1-1/n$ (by setting $\alpha = 1/n$ by crashing $\Theta(\sqrt{r_t\log n})$ processes using randomness in round $t$. If $r_t$ is very small, say $\sqrt{r_t\log n}>r_t$, simply all $r_t$ processes are crashed.

Consider an execution $\cE$ of the algorithm -- it is a random event generated dynamically when running the algorithm against some adaptive adversary's strategy.
Let us restrict the adversary to strategies in which it can crash at most $\Theta(\sqrt{r_t\log n})$ processes in a round $t\le \tau$, where $r_t$ denotes the number of processes using randomness in round $t$. From now on, by `adversary' we will mean the restricted one.




For any round $t\le \tau$, let: 
\begin{itemize}
    \item 
$\cE_t$ be an execution of the algorithm by round $t$, 
\item
$\cA_t$ be an adversarial strategy possible after round $t$ under the history $\cE_t$,
\item
$\cP(\cE_t,\cA)$ be the probability of reaching consensus in value $1$ when continue the run of the algorithm with history $\cE_t$ under adversarial strategy $\cA$. 
\end{itemize}
%
\paragraph{Types of executions.}
Following classic terminology in distributed computing~\cite{AW}, we say that an execution 
%state of the algorithm in round $t$, defined uniquely by its history 
$\cE_t$ is:
\begin{itemize}
    \item 
{\em null-valent} if for all adversarial strategies $\cA$ we have $\frac{1}{\tau\log n} + \frac{t}{n} \le \cP(\cE_t,\cA)\le 1-\frac{1}{\tau\log n} + \frac{t}{n}$,
\item
{\em $1$-valent} if there is adversarial strategy $\cA$ such that $\cP(\cE_t,\cA)> 1-\frac{1}{\tau\log n} + \frac{t}{n}$ and for every other adversarial strategy $\cA'$: $\frac{1}{\tau\log n} + \frac{t}{n} \le \cP(\cE_t,\cA')$,
\item
{\em $0$-valent} if there is adversarial strategy $\cA$ such that $\cP(\cE_t,\cA) < \frac{1}{\tau\log n} + \frac{t}{n}$ and for every other adversarial strategy $\cA'$: $\cP(\cE_t,\cA') \le 1- \frac{1}{\tau\log n} + \frac{t}{n}$,
\item
{\em bi-valent} if there are adversarial strategies $\cA,\cA'$ such that $\cP(\cE_t,\cA)> 1-\frac{1}{\tau\log n} + \frac{t}{n}$ and $\cP(\cE_t,\cA') < \frac{1}{\tau\log n} + \frac{t}{n}$.
\end{itemize}

An execution that is $1$-valent or $0$-valent is also called {\em uni-valent}. 


\paragraph{Starting executions.}
In \cite{Bar-JosephB98}, the authors proved that an adaptive adversary could turn some initial execution, which is in fact a vector of initial values ot processes, into a null-valent or bi-valent execution by crashing at most one process.
Although in their analysis they assumed only the case of $\tau=\Theta(\sqrt{n})$, that particular result holds for any $\tau < n$, i.e., when the probabilistic thresholds in the definitions of null-valent and bi-valent executions should be strictly in $(0,1)$.
This result holds even if the algorithm can use unlimited randomness and communication, therefore it automatically applies in our case of restricted randomness and our considered range of $\tau$. More precisely:

%We start from citing a result regarding existing of a ``bad'' initial state, i.e., such that an adaptive adversary could turn it into null-valent or bi-valent. It was proved even if the algorithm can use unlimited randomness and communication, therefore it automatically applies in our case of restricted randomness.

\begin{lemma}[Lemma 3.5 in~\cite{Bar-JosephB98}]
\label{lem:lower-initial}
Any synchronous Consensus algorithm has an initial state which by crashing at most one process becomes null-valent or bi-valent.
\end{lemma}

It follows from Lemma~\ref{lem:lower-initial} that it is sufficient to consider executions starting from bi-valent or null-valent executions.

\paragraph{Extending null-valent executions.}
The following lemma provides an argument to extend null-valent execution at round $t<\tau$ to a null-valent execution in round $t+1$. This way, starting from a null-valent execution, the adversary could keep extending it until a null-valent execution at round~$\tau$.

\begin{lemma}
\label{lem:lower-null}
A null-valent execution $\cE_t$ could be extended to a null-valent execution $\cE_{t+1}$ with probability at least $1-1/n$.
\end{lemma}

\begin{proof}
The proof follows directly from Lemma 3.1 in~\cite{Bar-JosephB98}, by replacing their specific Corollary 2.2 by our generalized version applied to $r_t$ processes that use randomness.
\end{proof}

\paragraph{Extending bi-valent executions.}


\paragraph{Bounding randomness.}

Consider the total amount of randomness used (i.e., the sum over all processes $p$ and rounds $t$ such that process $p$ uses randomness in round $t$):
\[
\sum_{t\le \tau} r_t
\]
and assume, by contradiction, that it is asymptotically smaller than $n\cdot \frac{n}{\tau\log n} = \frac{n^2}{\tau\log n}$. It follows that the adversary has crashed asymptotically at most
\[
\sum_{t\le \tau} \sqrt{r_t\log n}
\le
\sqrt{\tau\sum_{t\le \tau} (r_t\log n) }
<<
n
%\sqrt{\log n} \sum_{t\le \tau} \sqrt{r_t}
\]
processes by round $\tau$, by Cauchy-Schwarz Inequality and the (contradictory) assumption.
It means that the adversary can still continue crashing processes and enforce the system to be in null-valent state, by Lemma~\ref{lem:lower-null}, which is a contradiction.


==> src/proofs-gossip.tex <==
\section{Skipped proofs of Lemmas and Theorems from Section~\ref{sec:goss-fuz-cnt-short}} \label{sec:gossip-long}

==> src/proofs-param-consensus.tex <==
\section{Skipped proofs of Lemmas and Theorems from Section~\ref{sec:param-short}}

\begin{lemma*}[Lemma~\ref{lem:phase-1-sync-comm} in the main part.]
For every $i \in [x]$, there is at most one iteration of the main loop in which $SP_{i}$ communicates with any other super-processor.
\end{lemma*}
\begin{proof}
Let us fix any super-processor $SP_{i}$ and consider the \textit{first} round $r$ in which that super-processors communicates with another one. If such round does not exist the lemma holds. Now, if a member $p$ of the super-processor $SP_{i}$ executes line~\ref{alg:phase-1:direct-comm} it must have its variables $\texttt{is\_active}$ and $\texttt{candidate\_value}$ set to $\texttt{true}$ and $1$ respectively. In particular this means, that $p$ had to execute line~\ref{alg:phase-1:first-stable} before it reached line~\ref{alg:phase-1:direct-comm} in this iteration. Otherwise, its value $\texttt{candidate\_value}$ would be $0$. This, let us conclude that the $\frac{2}{3}$ $\text{-stable-}\textsc{GroupConsensus}$ algorithm executed in line~\ref{alg:phase-1:first-stable} returned value $1$. Since we used a Consensus algorithm with the $\frac{3}{3}$-stability property, see Theorem~\ref{thm:stable-cons}, we have that at least $\frac{2}{3}|SP_{i}|$ members started the synchronous execution of line~\ref{alg:phase-1:first-stable}. It easily follows, that each of this members either became faulty or executed line~\ref{alg:phase-1:direct-comm} later in the same iteration of the main loop. If a member executed line~\ref{alg:phase-1:direct-comm} it will set its variable \texttt{is\_active} to \texttt{false} and will be idle for the rest of the algorithm run, in particular will not participate in any future run of the $\frac{2}{3}$ $\text{-stable-}\textsc{GroupConsensus}$ algorithm. The same holds if a member became a faulty process. It gives us that at most $\frac{1}{3}|SP_{i}|$ members of $SP_{i}$ can participate with value other than $0$. Since they always execute the $\frac{2}{3}$-stable Consensus, thus according to Theorem~\ref{thm:stable-cons}, the result will always be $0$. This proves that $SP_{i}$ will not communicate in any other round than $r$. 
\end{proof}


==> src/proofs-rand-consensus.tex <==
\section{Pseudocode of the \textsc{GroupConsensus} algorithm} \label{sec:group-long}

\begin{algorithm}[H]\label{fig:group-cons}
%\SetAlgorithmName{ParamConsensus}
\SetAlgoLined
\SetKwInput{Input}{input}
\SetKwInput{Output}{output}
\Input{$\cP$, $p$, $b_{p}$}
\Output{a consensus value}
$r:=1$; $N_{-1}^r = N_0^r = n$; $b_p = x_p$; $\texttt{decided} = FALSE$ \;
\While{$TRUE$}
{
	\ul{participate in \textsc{CheapCounting} execution with input bit being set to $b_p$; let $O_p^r$, $Z_p^r$ be the numbers of ones and zeros (resp.) returned by \textsc{CheapCounting}}\;
	$N_p^r = Z_p^r + O_p^r$\;
	\If{$(N_p^r < \sqrt{n/ \log n })$}
	{
	    send $b_p$ to all processes, receive all messages sent to $p$ in round $r+1$\;
	    implement a deterministic protocol for $\sqrt{n/ \log n}$ rounds\;
	}
	\If{$\texttt{decided} = TRUE$}
	{
	    \texttt{diff} $=$ $N_p^{r-3}$ $N_i^r$\;
        \lIf{(\texttt{diff} $\leq N_p^{r-2}/10$)}{STOP}
        \lElse{\texttt{decided} $= FALSE$}
	}
	\lIf{$O_p^r > (7N_p^r-1)/10$}{$b_p = 1$, decided $= TRUE$}
	\lElseIf{$O_p^r > (6N_p^r-1)/10$}{$b_p = 1$}
	\lElseIf{$Z_p^r = 0$}{$b_p = 1$}
	\lElseIf{$O_p^r < (4N_p^r-1)/10$}{$b_p = 0$, decided $= TRUE$}
	\lElseIf{$O_p^r < (5N_p^r-1)/10$}{$b_p = 0$}
	\lElse{set $b_p$ to $0$ or $1$ with equal probability}
	
    $r := r + 1$\;
}

\Return{$b_{p}$}
\caption{\textsc{GroupConsensus}. The part in which our algorithm differs from the \textsc{SynRyn} algorithm from~\cite{Bar-JosephB98} algorithm is underlined.}
\end{algorithm}
